Augmenting semantic lexicons using word embeddings and transfer learning

Sentiment-aware intelligent systems are essential to a wide array of applications. These systems are driven by language models which broadly fall into two paradigms: Lexicon-based and contextual. Although recent contextual models are increasingly dominant, we still see demand for lexicon-based models because of their interpretability and ease of use. For example, lexicon-based models allow researchers to readily determine which words and phrases contribute most to a change in measured sentiment. A challenge for any lexicon-based approach is that the lexicon needs to be routinely expanded with new words and expressions. Here, we propose two models for automatic lexicon expansion. Our first model establishes a baseline employing a simple and shallow neural network initialized with pre-trained word embeddings using a non-contextual approach. Our second model improves upon our baseline, featuring a deep Transformer-based network that brings to bear word definitions to estimate their lexical polarity. Our evaluation shows that both models are able to score new words with a similar accuracy to reviewers from Amazon Mechanical Turk, but at a fraction of the cost.

==> bin/countcheckboxes-total <==
#!/usr/bin/perl

undef $/;
    $counts=0;
foreach $file (@ARGV) {
    open (FILE, "$file") or die "can't open $file: $!\n";

    $text = <FILE>;
    while ($text =~ m/\\todo{/g) {
	$counts++;
    }
    close FILE;
}
print "$counts";


==> bin/rename <==
#!/usr/bin/perl

$usage = "rename text1 text2 file [files...]

swap text1 for text2 in file names
whenever text1 is found.

swaps only the first instance.

rudimentary first version: use only for static text.
";

$pattern1 = $ARGV[0];
$pattern2 = $ARGV[1];

foreach $filename (@ARGV[2..$#ARGV]) {
    if ($filename =~ m/$pattern1/) {
	($newfilename = $filename) =~ s/$pattern1/$pattern2/g;
	print "renaming $filename as $newfilename...\n";
	`mv "$filename" "$newfilename"`;
    }
}


==> extra_intro.tex <==
Building  on  the  recent  models  discussed  above,  we  develop framework for augmenting semantic dictionaries using word embeddings and transfer learning.
[YOU CAN ADD THE PARAGRAPH BELOW TO THE SENTENCE ABOVE THAT IS CURRENTLY IN RELATED WORK.]
There have been a number of studies in automatic lexicon generators, but the general overlying assumption is that words that co-occur together have similar sentiment polarity. One method is to use seed words of known polarity and measure co-occurrence in selected corpora using pointwise mutual information~\cite{turney_Measuring_2003, kiritchenko_Sentiment_2014}. Another approach is to use a word graph such as WordNet~\cite{fellbaum_WordNet_1998}, which maps words that are related in meaning, and uses proximity in the graph to seed words of known sentiment to generate sentiment scores~\cite{baccianella_SentiWordNet_2010, qiu_Expanding_2009, sanvicente_Simple_2014}. Recently, word embeddings, which essentially look at word co-occurrence, have also been used to generate sentiment lexicons~\cite{tang_Building_2014, wang_CommunityBased_2016, ljubesic_Predicting_2018, thavareesan_Sentiment_2020}. In terms of approach, our model is closest to~\citet{amir_INESCID_2015, li_Inferring_2017}, where traditional regression models are trained on word embeddings and known sentiment scores. In contrast, we use deep learning models that ... (NOTE: I think you're in a better position to explain this). Further, while some of these models only predict sentiment polarity~\cite{alshari_Effective_2018,thavareesan_Sentiment_2020}, ours predict sentiment scores. More details on previous work on automatic sentiment lexicon generation can be found in~\cite{darwich_CorpusBased_2019}.

==> make-arxiv-submission <==
#!/usr/bin/perl
$usage = "make-arxiv-submission foo as in foo-revtex4.tex\n";

$basefilename = $ARGV[0];

print "making a single latex file...\n";
`make-single-latex-file.pl $basefilename-revtex4.tex`;
print "finding figures and linking...\n";
`makelinks.pl $basefilename-revtex4-combined.tex`;
print "making package...\n";
`makepackage $basefilename`;



==> sentiment-analysis-revtex4.settings.tex <==
\newcommand{\filenamebase}{sentiment-analysis}


==> sentiment-analysis.nutshell.tex <==
\todo{Write a 1--3 sentence nutshell (logline)}



==> sentiment-analysis.outtakes.tex <==

Sentiment-aware intelligent systems are essential to an enormous set of applications from 
marketing and political campaigns 
to recommender systems 
to behavioral and social psychology 
to intelligence and national security.
These sentiment-aware intelligent systems are driven by language models, 
which fall into two paradigms: 
Lexicon-based or contextual.
Although recent contextual models are relevant to a wide range of applications,
we still see demand for lexicon-based models 
because of their interpretability and ease of use.
For example, 
lexicon-based models allow
researchers to determine
which words contribute most to a change in sentiment.
Sentiment lexicons
need to be updated periodically 
to support new words and expressions.
Crowdsourcing annotations 
for semantic dictionaries may be an expensive and time-consuming task.
Here, 
we propose two models for predicting sentiment scores to augment semantic lexicons 
at a relatively low cost using word embeddings and transfer learning.
Our first model establishes a baseline employing a simple and shallow neural network 
initialized with pre-trained word embeddings using a non-contextual approach.
Our second model improves upon our baseline, featuring a deep Transformer-based network 
that brings to bear word definitions to estimate their lexical polarity.
Our evaluation shows that both models are able to score new words 
with a similar accuracy to reviewers from Amazon Mechanical Turk, 
but at a fraction of the cost.



%\paragraphnutshell{Sentiment analysis schemes}

The body of research in this domain continues to flourish, leading to the development of an enormous number of sentiment analysis methods.
Methodologically, these tools can be categorized into two major schemes:
sentiment classification and sentiment scoring.
Though most applications of sentiment analysis frame the task as binary classification
(i.e., positive and negative),
researchers argue that the addition of a neutral class improves the overall performance of the system,
particularly for edge cases~\cite{ribeiro2016sentibench}.
Others emphasize the importance of sentiment scoring,
whereby we adopt a scaling system to gauge the polarity of emotions in a piece of text~\cite{thelwall2010sentiment}.
The sentiment scoring paradigm is widely adopted in e-commerce, movies, and restaurant reviews~\cite{snyder2007multiple}.



%\paragraphnutshell{Sentiment-aware intelligent systems}

Starting with the marketing industry,
evaluating consumer feedback regarding a product or service helps business owners to make informed decisions regarding product development and risk management~\cite{cabral2010dynamics,turney2002thumbs}.
Movie creators and producers---among many others in the entertainment
industry---leverage these tools to gauge movie ratings and reviews~\cite{pang2002thumbs}.
Augmenting online recommendation systems with sentiment rating
along with similarity ranking further improves the user experience~\cite{terveen1997phoaks,tang2009survey}.

Over the past decade, 
we have seen tremendous efforts among the NLP community,
developing end-to-end models to examine short- and medium-length texts~\cite{wilson2005recognizing,feldman2013techniques},
particularly for social media~\cite{pak2010twitter,agarwal2011sentiment,korkontzelos2016analysis}.


Analyzing sentiment of online political discourse 
provides an understanding of public support or opposition on pending policies, 
giving policymakers an important window into the public's awareness and attitude~\cite{laver2003extracting,thomas2006get}. 
Beyond that, 
these tools can also forecast elections~\cite{tumasjan2010predicting}, 
and monitor inflammatory discourse on social media, with vital relevance national security~\cite{pang2008opinion}.


Using the sentiment analysis techniques developed by the computational linguistics community,
researchers in clinical and behavioral psychology have gained a greater understanding of several public health issues~\cite{coppersmith2014quantifying,yadollahi2017current,gohil2018sentiment}.
Recent studies convey the utility of sentiment analysis tools
to examine the language used in discussions related to mental health on social media~\cite{bathina2021individuals,stupinski2021quantifying},
especially in light of the latest advances in NLP and emerging ethical concerns~\cite{conway2016social}.


%\paragraphnutshell{Sentiment analysis paradigms}

Most sentiment analysis tasks have a similar structure, 
whereby a model takes in a piece of text and outputs a sentiment score or a probability of belonging to a specific class 
(e.g., positive, negative, or neutral).
While many terms have been used to describe the process of automatic distillation of lexical and emotional polarity of digitized text archives, 
models can be classified into one of two systematic paradigms: 
lexicon-based models and contextual language models.


%\paragraphnutshell{Lexicon-based models}

Lexicon-based models compute sentiment scores based on sentiment dictionaries that are usually constructed by human annotators~\cite{turney2002thumbs,taboada2011lexicon,augustyniak2016comprehensive}.
Most of these models use simple statistical methods (e.g., weighted average) 
to estimate sentiment for a given document or short text snippet.
Recent developments of large-scale lexicon dictionaries
(e.g., labMT~\cite{dodds2015human},
NRC-VAD~\cite{mohammad2018word,mohammad2018obtaining},
EPA~\cite{osgood1962studies},
and SocialSent~\cite{hamilton2016inducing})
have enabled tremendous studies across many disciplines.
Many examples for applying lexicon-based models
to explore and identify behavioral and linguistic patterns
of language and human nature can be readily seen
from quantifying happiness of digitized text archives~\cite{dodds2015human}
to examining short informal text~\cite{thelwall2010sentiment}
to gauging the hedonic tone of discourse on social media~\cite{dodds2011temporal}.


The simplicity of lexicon-based models,
however,
is a double-edged sword.
While the models are easily explainable,
the vast majority of these models gloss over context.
Consider the following two sentences:
``The dog is \textit{lying} on the beach.''
and
``I never said that, you are \textit{lying}!''.
The word `lying' has vastly different meanings in these examples.
A lexicon-based model will have a fixed sentiment score of that word, regardless of its context.

%\paragraphnutshell{Contextual models}

In contrast,
contextual language models can overcome that challenge
by extrapolating semantics based on the surrounding words.
Context-aware models are used for a wide range of canonical NLP tasks, such as
text generation,
text classification,
named-entity recognition,
and, of course, sentiment analysis.
Such models are trained in a supervised or semi-supervised fashion 
on large-scale and annotated datasets,
building upon classical machine learning methods, such as support vector machines or naive Bayes classifiers~\cite{wilson2005recognizing,pak2010twitter,agarwal2011sentiment,feldman2013techniques},
or recent advanced models powered by deep neural networks~\cite{socher2013recursive}.


%\paragraphnutshell{OOV challenge}
Although contextual models are widely used,
we still observe a consistent demand for lexicon-based models because of their 
simplicity, 
ease of use,
and ease of interpretability~\cite{pang2008opinion,taboada2011lexicon,dodds2015human}.
Researchers use word shifts to study how words contribute to sentiment shifts~\cite{dodds2011temporal,reagan2017sentiment,gallagher2021generalized}.


A big challenge in lexicon-based models
is the time and financial investment associated with maintaining them.
Lexicon dictionaries need to get updated regularly to mitigate the out-of-vocabulary
(OOV) problem---words/phrases that were not considered when the dictionaries were originally constructed~\cite{riloff1996empirical}.
While researchers show general sentiment trends are observable
unless the lexicon dictionary does not have enough words,
having a versatile dictionary with specialized and rarely used words improves the signal~\cite{dodds2010measuring}.
Notably,
language is an evolving sociotechnical phenomenon.
New words are often created in real-time,
especially on social media~\cite{alshaabi2021storywrangler}.
Words occasionally substitute others or drift in meaning over time.
For example,
the word `covid' slowly became the most narratively trending $n$-gram
in reference to the global Coronavirus outbreak during 2020~\cite{alshaabi2021world}.


